Quantifying the Performance Benefits of Partitioned Communication in MPI

Partitioned communication was introduced in MPI 4.0 as a user-friendly interface to support pipelined communication patterns, particularly common in the context of MPI+threads. It provides the user with the ability to divide a global buffer into smaller independent chunks, called partitions, which can then be communicated independently. In this work we first model the performance gain that can be expected when using partitioned communication. Next, we describe the improvements we made to \mpich{} to enable those gains and provide a high-quality implementation of MPI partitioned communication. We then evaluate partitioned communication in various common use cases and assess the performance in comparison with other MPI point-to-point and one-sided approaches. Specifically, we first investigate two scenarios commonly encountered for small partition sizes in a multithreaded environment: thread contention and overhead of using many partitions. We propose two solutions to alleviate the measured penalty and demonstrate their use. We then focus on large messages and the gain obtained when exploiting the delay resulting from computations or load imbalance. We conclude with our perspectives on the benefits of partitioned communication and the various results obtained.

==> figures/results/BW_sleep-4part-4thread-100sleep-1vci-0aggr.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkolivegreen9912157}{RGB}{99,121,57}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={msg size [\B]},
xmajorgrids,
xmin=16, xmax=67108864,
xmode=log,
xtick style={color=black},
xtick={1,10,100,1000,10000,100000,1000000,10000000,100000000,1000000000},
xticklabels={
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\),
  \(\displaystyle {10^{9}}\)
},
y grid style={darkgray176},
ylabel={bandwidth [\GBs]},
ymajorgrids,
ymin=0.00208215504622497, ymax=101.520940446324,
ymode=log,
ytick style={color=black},
ytick={0.0001,0.001,0.01,0.1,1,10,100,1000,10000},
yticklabels={
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\)
}
]
\addplot [thick, steelblue31119180]
table {%
32 0.00409818220005789
64 0.00836857287065586
128 0.0159604718962899
256 0.0268479659467112
512 0.053079656806844
1024 0.0902787267525666
2048 0.173709330345442
4096 0.34182527687764
8192 0.634607325097589
16384 1.50967735990749
32768 2.70119215823341
65536 4.19077704204142
131072 8.51012440680982
262144 17.9082249922975
524288 30.0581971663352
1048576 41.0154670104649
2097152 50.0621733333811
4194304 56.3399548802594
8388608 59.8987336348998
16777216 62.1530990758101
33554432 61.6811679454704
};
\addlegendentry{\ptpart{}}
\addplot [thick, darkorange25512714]
table {%
32 0.0203190084323885
64 0.0320147267743162
128 0.069929305842375
256 0.121241225995066
512 0.235232174615784
1024 0.457886923393371
2048 0.603373885282951
4096 1.11386889143123
8192 2.11251243280098
16384 2.1765604473108
32768 3.77833070609746
65536 6.53002009742819
131072 9.33082749587106
262144 13.1953515460031
524288 17.221180796318
1048576 20.2694432405871
2097152 22.2111839238694
4194304 23.3887470027324
8388608 24.0144098917999
16777216 24.3501947468001
33554432 24.2673262457511
};
\addlegendentry{\ptsingle{}}
\addplot [thick, darkolivegreen9912157]
table {%
32 0.00425463286307674
64 0.00855005381858095
128 0.0163843355511921
256 0.0280974102090184
512 0.0556697643483653
1024 0.0951475670005194
2048 0.182270459814615
4096 0.353142111248387
8192 0.647695943440458
16384 1.39714278161372
32768 2.59907341382995
65536 3.64581276156854
131072 7.39507442636436
262144 15.7898858090762
524288 28.6014326683516
1048576 40.1195425976678
2097152 49.3607109686755
4194304 56.0515444395459
8388608 59.9704173103773
16777216 62.1197532866358
33554432 61.7114792834984
};
\addlegendentry{\ptmany{}}
\addplot [thick, crimson2143940]
table {%
32 0.00340099434446525
64 0.00731161175341589
128 0.0144588868893704
256 0.0288736577837686
512 0.0542789173052214
1024 0.0801000624999511
2048 0.161288417239275
4096 0.319882792945397
8192 0.611610292553092
16384 1.46325692555287
32768 2.84216725661644
65536 5.76851644840498
131072 10.5066472146627
262144 21.3991957669193
524288 32.2292478358637
1048576 41.8381601002607
2097152 50.215309171711
4194304 56.1269635318938
8388608 59.7161481747247
16777216 61.7211506908177
33554432 60.5739740701814
};
\addlegendentry{\RMAsingle{}}
\draw[<->,draw=black,semithick] (axis cs:33554432,61.6811679454704) -- (axis cs:33554432,24.2673262457511);
\draw (axis cs:33554432,24.2673262457511) ++(-20pt,-10pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{$\times 2.5417$};
\end{axis}

\end{tikzpicture}


==> figures/results/TIME_aggr-32part-4thread-0sleep-1vci.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkolivegreen9912157}{RGB}{99,121,57}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={msg size [\B]},
xmajorgrids,
xmin=142.024892424684, xmax=60481894.7252872,
xmode=log,
xtick style={color=black},
xtick={10,100,1000,10000,100000,1000000,10000000,100000000,1000000000},
xticklabels={
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\),
  \(\displaystyle {10^{9}}\)
},
y grid style={darkgray176},
ylabel={time [\mus]},
ymajorgrids,
ymin=1, ymax=1913.62625976378,
ymode=log,
ytick style={color=black},
ytick={0.1,1,10,100,1000,10000,100000},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
}
]
\addplot [thick, black, dash pattern=on 12.8pt off 3.2pt on 2pt off 3.2pt, forget plot]
table {%
128000 5.12
131601.221226231 5.26404884904925
135303.76115809 5.4121504463236
139110.470350835 5.56441881403342
143024.279558792 5.72097118235169
147048.201991711 5.88192807966843
151185.335634614 6.04741342538458
155438.865632914 6.21755462531655
159812.066744621 6.39248266978485
164308.305861564 6.57233223446255
168931.044601523 6.75724178406091
173683.841973307 6.94735367893229
178570.357116805 7.1428142846722
183594.352120123 7.34377408480493
188759.694915992 7.55038779663968
194070.362259651 7.76281449038605
199530.442790525 7.98121771162101
205144.14018003 8.2057656072012
210915.776367946 8.43663105471784
216849.794889847 8.67399179559389
222950.764298138 8.91803057192552
229223.381679349 9.16893526717395
235672.476270381 9.42689905081525
242303.013176501 9.69212052706006
249120.097193932 9.96480388775727
256128.976739991 10.2451590695996
263335.047893811 10.5334019157524
270743.858550732 10.8297543420293
278361.11269358 11.1344445077432
286192.674784124 11.4477069913649
294244.574278065 11.7697829711226
302523.010267077 12.1009204106831
311034.35625143 12.4413742500572
319785.165046898 12.7914066018759
328782.173829717 13.1512869531887
338032.309323482 13.5212923729393
347542.693131981 13.9017077252792
357320.647222047 14.2928258888819
367373.699560693 14.6949479824277
377709.589910827 15.1083835964331
388336.27579003 15.5334510316012
399261.938596989 15.9704775438795
410494.989910283 16.4197995964113
422044.077964396 16.8817631185759
433918.094307917 17.3567237723167
446126.180649069 17.8450472259628
458677.735893843 18.3471094357537
471582.423382129 18.8632969352851
484850.178327452 19.3940071330981
498491.215466006 19.9396486186402
512516.036920896 20.5006414768358
526935.440287643 21.0774176115057
541760.526947153 21.6704210778861
557002.710612593 22.2801084245037
572673.726116707 22.9069490446683
588785.638446366 23.5514255378547
605350.852031314 24.2140340812526
622382.120294223 24.8952848117689
639892.555469461 25.5957022187785
657895.638698086 26.3158255479234
676405.230406871 27.0562092162748
695435.580979334 27.8174232391734
715001.341726984 28.6000536690794
735117.576169259 29.4047030467704
755799.771630793 30.2319908652317
777063.851164993 31.0825540465997
798926.18581306 31.9570474325224
821403.607207919 32.8561442883167
844513.420532764 33.7805368213106
868273.417844168 34.7309367137667
892701.891770049 35.708075670802
917817.649593013 36.7127059837205
943640.027729919 37.7456011091968
970188.906618846 38.8075562647538
997484.726024861 39.8993890409944
1025548.50077644 41.0219400310577
1054401.83694461 42.1760734777845
1084066.94847728 43.3626779390914
1114566.6743016 44.582666972064
1145924.49590742 45.8369798362968
1178164.55542555 47.1265822170218
1211311.67421455 48.4524669685818
1245391.37197051 49.8156548788203
1280429.88637446 51.2171954549784
1316454.19329253 52.658167731701
1353492.02754445 54.1396811017781
1391571.90425639 55.6628761702555
1430723.14081447 57.228925632579
1470975.87943605 58.839035177442
1512361.11037589 60.4944444150355
1554910.69578536 62.1964278314144
1598657.39424283 63.9462957697133
1643634.88597423 65.7453954389693
1689877.79878317 67.595111951327
1737421.73471063 69.4968693884254
1786303.29744466 71.4521318977866
1836560.12050126 73.4624048200505
1888230.89619813 75.5292358479252
1941355.40544356 77.6542162177423
1995974.54836342 79.8389819345367
2052130.37578985 82.0852150315941
2109866.12163586 84.3946448654343
2169226.23618072 86.7690494472286
2230256.4202919 89.210256811676
2293003.66060982 91.7201464243928
2357516.26572243 94.3006506288973
2423843.90335763 96.9537561343051
2492037.63862202 99.681505544881
2562149.97331557 102.485998932623
2634234.88635222 105.369395454089
2708347.87531793 108.333915012717
2784545.99919772 111.381839967909
2862887.92230498 114.515516892199
2943433.95944659 117.737358377864
3026246.12235884 121.049844894354
3111388.16744978 124.455526697991
3198925.64488466 127.957025795386
3288925.94905258 131.557037962103
3381458.37045283 135.258334818113
3476594.14904105 139.063765961642
3574406.52907635 142.976261163054
3674970.81551142 146.998832620457
3778364.43196924 151.13457727877
3884666.98035084 155.386679214034
3993960.30212021 159.758412084808
4106328.54131334 164.253141652534
4221858.20932004 168.874328372802
4340638.25148833 173.625530059533
4462760.1156028 178.510404624112
4588317.82228943 183.532712891577
4717408.03740133 188.696321496053
4850130.14644105 194.005205857642
4986586.33107658 199.463453243063
5126881.64781024 205.075265912409
5271124.10886078 210.844964354431
5419424.76532117 216.776990612847
5571897.79265584 222.875911706234
5728660.57860353 229.146423144141
5889833.81355307 235.593352542123
6055541.58346201 242.22166333848
6225911.46538926 249.036458615571
6401074.6257158 256.042985028632
6581165.92112845 263.246636845138
6766324.00244499 270.6529600978
6956691.42136033 278.267656854413
7152414.74019584 286.096589607833
7353644.64473648 294.145785789459
7560536.06024264 302.421442409706
7773248.2707257 310.929930829028
7991945.04157965 319.677801663186
8216794.74566254 328.671789826501
8447970.49292555 337.918819717022
8685650.26368883 347.426010547553
8930017.04566709 357.200681826684
9181258.9748504 367.250358994016
9439569.48034852 377.582779213941
9705147.43331038 388.205897332415
9978197.30003336 399.127892001334
10258929.2993803 410.35717197521
10547559.5646251 421.902382585003
10844310.3098521 433.772412394086
11149410.0010371 445.976400041485
11463093.531941 458.523741277639
11785602.4049527 471.424096198108
12117184.9170202 484.687396680807
12458096.3508119 498.323854032477
12808599.1712571 512.343966850284
13168963.2276151 526.758529104602
13539465.9612303 541.57863844921
13920392.619132 556.815704765279
14312036.4736436 572.481458945745
14714699.0481708 588.587961926833
15128690.3493418 605.147613973671
15554329.1056788 622.17316422715
15991943.0129846 639.677720519385
16441868.9866334 657.674759465337
16904453.4209583 676.178136838331
17380052.4559379 695.202098237516
17869032.2513858 714.761290055433
18371769.2688538 734.870770754154
18888650.5614665 755.54602245866
19420074.0719104 776.802962876415
19966448.9388069 798.657957552275
20528195.8117045 821.127832468181
21105747.1749337 844.22988699735
21699547.6805731 867.981907222925
22310054.4907833 892.402179631332
22937737.6297722 917.50950519089
23583080.3456633 943.323213826533
24246579.482544 969.86317930176
24928745.8629818 997.149834519272
25630104.6813029 1025.20418725211
26351195.9079344 1054.04783631738
27092574.7051238 1083.70298820495
27854811.8543531 1114.19247417412
28638494.1957794 1145.53976783118
29444225.0800384 1177.76900320154
30272624.8327584 1210.90499331034
31124331.2321449 1244.97324928579
32000000 1280
};
\addplot [thick, steelblue31119180]
table {%
256 26.79919
512 26.96461
1024 26.60731
2048 33.41948
4096 32.25287
8192 32.70859
16384 37.61425
32768 39.68891
65536 44.0736
131072 50.91393
262144 58.81639
524288 99.21641
1048576 99.10033
2097152 101.8244
4194304 183.8109
8388608 354.0859
16777216 694.0098
33554432 1384.324
};
\addlegendentry{\ptpart{}}
\addplot [thick, steelblue31119180, dash pattern=on 2pt off 3.3pt]
table {%
256 6.768987
512 7.043593
1024 9.526567
2048 12.31963
4096 14.67854
8192 20.04014
16384 37.25018
32768 39.74425
65536 44.21993
131072 51.65333
262144 59.63169
524288 94.96862
1048576 93.50427
2097152 101.6185
4194304 184.359
8388608 354.1218
16777216 694.0826
33554432 1382.203
};
\addlegendentry{\ptpart{}~(aggr = $512$\B)}
\addplot [thick, steelblue31119180, dash pattern=on 12.8pt off 3.2pt on 2pt off 3.2pt]
table {%
256 6.820733
512 6.908187
1024 6.91394
2048 9.361673
4096 12.11053
8192 14.83741
16384 21.07325
32768 38.75932
65536 42.93399
131072 50.80553
262144 59.01826
524288 94.39877
1048576 94.78541
2097152 101.0454
4194304 183.5881
8388608 353.9975
16777216 693.8238
33554432 1384.526
};
\addlegendentry{\ptpart{}~(aggr = $1024$\B)}
\addplot [thick, steelblue31119180, dash pattern=on 7.4pt off 3.2pt]
table {%
256 6.94234
512 6.972593
1024 6.949407
2048 7.548347
4096 8.72524
8192 10.20092
16384 12.97025
32768 16.26544
65536 26.75229
131072 51.30094
262144 57.17123
524288 95.42987
1048576 93.91524
2097152 101.3308
4194304 183.9244
8388608 354.2886
16777216 693.9953
33554432 1383.273
};
\addlegendentry{\ptpart{}~(aggr = $4096$\B)}
\addplot [thick, steelblue31119180]
table {%
256 6.74866
512 7.161413
1024 7.0248
2048 8.05754
4096 8.984707
8192 9.2085
16384 11.28898
32768 13.67801
65536 18.88086
131072 28.87425
262144 50.13504
524288 95.82577
1048576 94.8562
2097152 101.4626
4194304 183.8268
8388608 353.4779
16777216 693.4146
33554432 1385.269
};
\addlegendentry{\ptpart{}~(aggr = $16384$\B)}
\addplot [thick, darkorange25512714]
table {%
256 2.163087
512 2.336167
1024 2.350747
2048 3.285707
4096 3.677853
8192 4.00004
16384 7.494473
32768 8.611407
65536 10.04163
131072 14.03413
262144 20.01167
524288 30.55292
1048576 51.79945
2097152 94.47019
4194304 179.3487
8388608 349.1959
16777216 688.978
33554432 1380.722
};
\addlegendentry{\ptsingle{}}
\addplot [thick, darkolivegreen9912157]
table {%
256 32.07206
512 32.10231
1024 31.91957
2048 39.44498
4096 39.11776
8192 38.50157
16384 42.55104
32768 43.58241
65536 47.78469
131072 55.05215
262144 64.65585
524288 102.2162
1048576 103.3774
2097152 105.7159
4194304 183.0703
8388608 353.0483
16777216 693.0774
33554432 1381.359
};
\addlegendentry{\ptmany{}}
\draw[->,draw=black,semithick] (axis cs:256,2.163087) -- (axis cs:256,6.768987);
\draw (axis cs:256,3.82647458934056) ++(2pt,-2pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{$\times 3.13$};

\draw[->,draw=black,semithick,dashed] (axis cs:256,27.79919) to[bend right, bend left] (axis cs:260,60);
\draw (axis cs:260,60) ++(2pt,-2pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{no aggr.};

\draw[->,draw=black,semithick] (axis cs:16384,38.25018) to[bend right, bend left] (axis cs:10384,150);
\draw (axis cs:10384,150) ++(2pt,-2pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{$32 \times 512$};

\draw[->,draw=black,semithick] (axis cs:131172,51.30094) to[bend right, bend left] (axis cs:132172,150);
\draw (axis cs:132172,150) ++(2pt,-2pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{$32 \times 4096$};
\end{axis}

\end{tikzpicture}


==> figures/results/TIME_congestion-32part-32thread-0sleep-1vci-0aggr.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkolivegreen9912157}{RGB}{99,121,57}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={msg size [\B]},
xmajorgrids,
xmin=142.024892424684, xmax=60481894.7252872,
xmode=log,
xtick style={color=black},
xtick={10,100,1000,10000,100000,1000000,10000000,100000000,1000000000},
xticklabels={
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\),
  \(\displaystyle {10^{9}}\)
},
y grid style={darkgray176},
ylabel={time [\mus]},
ymajorgrids,
ymin=1, ymax=2419.36321698645,
ymode=log,
ytick style={color=black},
ytick={0.1,1,10,100,1000,10000,100000},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.4]
(axis cs:256,142.536524)
--(axis cs:256,130.919076)
--(axis cs:512,124.097327)
--(axis cs:1024,126.103355)
--(axis cs:2048,145.040724)
--(axis cs:4096,143.183113)
--(axis cs:8192,147.739914)
--(axis cs:16384,149.705573)
--(axis cs:32768,155.171279)
--(axis cs:65536,163.95859)
--(axis cs:131072,175.491163)
--(axis cs:262144,194.498895)
--(axis cs:524288,239.273438)
--(axis cs:1048576,236.804949)
--(axis cs:2097152,237.908884)
--(axis cs:4194304,236.388725)
--(axis cs:8388608,360.38589)
--(axis cs:16777216,705.6535627)
--(axis cs:33554432,1429.5854817)
--(axis cs:33554432,1431.0985183)
--(axis cs:33554432,1431.0985183)
--(axis cs:16777216,706.1600373)
--(axis cs:8388608,386.59711)
--(axis cs:4194304,241.693475)
--(axis cs:2097152,243.606316)
--(axis cs:1048576,242.334851)
--(axis cs:524288,245.104162)
--(axis cs:262144,200.048705)
--(axis cs:131072,181.028637)
--(axis cs:65536,169.73261)
--(axis cs:32768,161.244921)
--(axis cs:16384,156.056427)
--(axis cs:8192,154.181686)
--(axis cs:4096,149.649687)
--(axis cs:2048,151.519076)
--(axis cs:1024,132.459845)
--(axis cs:512,130.348273)
--(axis cs:256,142.536524)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.4]
(axis cs:256,4.7207725)
--(axis cs:256,4.4675615)
--(axis cs:512,5.1314147)
--(axis cs:1024,5.10504465)
--(axis cs:2048,5.9327946)
--(axis cs:4096,6.3043057)
--(axis cs:8192,6.88314)
--(axis cs:16384,9.4371576)
--(axis cs:32768,10.7116044)
--(axis cs:65536,11.8311551)
--(axis cs:131072,16.8274042)
--(axis cs:262144,22.5074447)
--(axis cs:524288,32.4194858)
--(axis cs:1048576,54.4991326)
--(axis cs:2097152,100.383107)
--(axis cs:4194304,190.5277388)
--(axis cs:8388608,362.581858)
--(axis cs:16777216,700.7308607)
--(axis cs:33554432,1384.4320575)
--(axis cs:33554432,1385.3159425)
--(axis cs:33554432,1385.3159425)
--(axis cs:16777216,701.4421393)
--(axis cs:8388608,363.208542)
--(axis cs:4194304,191.0880612)
--(axis cs:2097152,100.615093)
--(axis cs:1048576,54.8432874)
--(axis cs:524288,32.6554342)
--(axis cs:262144,22.7954153)
--(axis cs:131072,17.1384158)
--(axis cs:65536,12.1537849)
--(axis cs:32768,10.9639156)
--(axis cs:16384,9.7374024)
--(axis cs:8192,7.143246)
--(axis cs:4096,6.5218543)
--(axis cs:2048,6.1770054)
--(axis cs:1024,5.25062135)
--(axis cs:512,5.4313853)
--(axis cs:256,4.7207725)
--cycle;

\path [draw=darkolivegreen9912157, fill=darkolivegreen9912157, opacity=0.4]
(axis cs:256,133.8675878)
--(axis cs:256,131.9154122)
--(axis cs:512,130.9423378)
--(axis cs:1024,130.9831793)
--(axis cs:2048,146.636143)
--(axis cs:4096,141.940044)
--(axis cs:8192,142.522438)
--(axis cs:16384,144.406114)
--(axis cs:32768,148.659089)
--(axis cs:65536,162.381122)
--(axis cs:131072,184.268294)
--(axis cs:262144,230.743271)
--(axis cs:524288,290.308881)
--(axis cs:1048576,286.239213)
--(axis cs:2097152,283.776238)
--(axis cs:4194304,284.760531)
--(axis cs:8388608,367.7053679)
--(axis cs:16777216,707.3840237)
--(axis cs:33554432,1514.61995)
--(axis cs:33554432,1517.22405)
--(axis cs:33554432,1517.22405)
--(axis cs:16777216,708.9221763)
--(axis cs:8388608,369.2448321)
--(axis cs:4194304,290.043669)
--(axis cs:2097152,288.890762)
--(axis cs:1048576,291.825987)
--(axis cs:524288,296.630319)
--(axis cs:262144,235.629529)
--(axis cs:131072,191.162106)
--(axis cs:65536,167.321878)
--(axis cs:32768,152.284711)
--(axis cs:16384,147.089086)
--(axis cs:8192,144.830962)
--(axis cs:4096,144.851156)
--(axis cs:2048,149.793457)
--(axis cs:1024,132.6842207)
--(axis cs:512,132.6534622)
--(axis cs:256,133.8675878)
--cycle;

\path [draw=orchid227119194, fill=orchid227119194, opacity=0.4]
(axis cs:256,110.590744)
--(axis cs:256,108.874056)
--(axis cs:512,108.1513257)
--(axis cs:1024,109.8757211)
--(axis cs:2048,109.1932441)
--(axis cs:4096,118.8551154)
--(axis cs:8192,123.2048155)
--(axis cs:16384,122.9924328)
--(axis cs:32768,124.93863)
--(axis cs:65536,129.484681)
--(axis cs:131072,155.550021)
--(axis cs:262144,186.868531)
--(axis cs:524288,193.689726)
--(axis cs:1048576,261.960205)
--(axis cs:2097152,325.9617659)
--(axis cs:4194304,432.15971)
--(axis cs:8388608,610.916406)
--(axis cs:16777216,952.826651)
--(axis cs:33554432,1777.357078)
--(axis cs:33554432,1792.784922)
--(axis cs:33554432,1792.784922)
--(axis cs:16777216,969.297349)
--(axis cs:8388608,612.939194)
--(axis cs:4194304,434.19049)
--(axis cs:2097152,327.3450341)
--(axis cs:1048576,264.583595)
--(axis cs:524288,197.521474)
--(axis cs:262144,190.944269)
--(axis cs:131072,159.714579)
--(axis cs:65536,131.755719)
--(axis cs:32768,126.61357)
--(axis cs:16384,124.0611672)
--(axis cs:8192,124.5399845)
--(axis cs:4096,120.0632846)
--(axis cs:2048,110.3819559)
--(axis cs:1024,111.0926789)
--(axis cs:512,109.5642743)
--(axis cs:256,110.590744)
--cycle;

\path [draw=crimson2143940, fill=crimson2143940, opacity=0.4]
(axis cs:256,40.7672167)
--(axis cs:256,40.1780033)
--(axis cs:512,40.1266959)
--(axis cs:1024,41.5312713)
--(axis cs:2048,41.6380535)
--(axis cs:4096,49.4750946)
--(axis cs:8192,51.9880462)
--(axis cs:16384,53.8307629)
--(axis cs:32768,56.5215289)
--(axis cs:65536,61.928403)
--(axis cs:131072,72.545267)
--(axis cs:262144,107.977208)
--(axis cs:524288,72.44395)
--(axis cs:1048576,71.554109)
--(axis cs:2097152,96.0740565)
--(axis cs:4194304,180.1742442)
--(axis cs:8388608,350.6840386)
--(axis cs:16777216,691.9624043)
--(axis cs:33554432,1511.523783)
--(axis cs:33554432,1513.884217)
--(axis cs:33554432,1513.884217)
--(axis cs:16777216,692.4641957)
--(axis cs:8388608,350.9941614)
--(axis cs:4194304,180.5477558)
--(axis cs:2097152,96.6954435)
--(axis cs:1048576,74.047331)
--(axis cs:524288,75.70883)
--(axis cs:262144,112.886592)
--(axis cs:131072,75.507833)
--(axis cs:65536,64.273257)
--(axis cs:32768,58.2723711)
--(axis cs:16384,55.4026171)
--(axis cs:8192,53.6051338)
--(axis cs:4096,51.0461254)
--(axis cs:2048,42.3088865)
--(axis cs:1024,42.2263487)
--(axis cs:512,40.8123641)
--(axis cs:256,40.7672167)
--cycle;

\addplot [thick, black, dash pattern=on 12.8pt off 3.2pt on 2pt off 3.2pt, forget plot]
table {%
128000 5.12
131601.221226231 5.26404884904925
135303.76115809 5.4121504463236
139110.470350835 5.56441881403342
143024.279558792 5.72097118235169
147048.201991711 5.88192807966843
151185.335634614 6.04741342538458
155438.865632914 6.21755462531655
159812.066744621 6.39248266978485
164308.305861564 6.57233223446255
168931.044601523 6.75724178406091
173683.841973307 6.94735367893229
178570.357116805 7.1428142846722
183594.352120123 7.34377408480493
188759.694915992 7.55038779663968
194070.362259651 7.76281449038605
199530.442790525 7.98121771162101
205144.14018003 8.2057656072012
210915.776367946 8.43663105471784
216849.794889847 8.67399179559389
222950.764298138 8.91803057192552
229223.381679349 9.16893526717395
235672.476270381 9.42689905081525
242303.013176501 9.69212052706006
249120.097193932 9.96480388775727
256128.976739991 10.2451590695996
263335.047893811 10.5334019157524
270743.858550732 10.8297543420293
278361.11269358 11.1344445077432
286192.674784124 11.4477069913649
294244.574278065 11.7697829711226
302523.010267077 12.1009204106831
311034.35625143 12.4413742500572
319785.165046898 12.7914066018759
328782.173829717 13.1512869531887
338032.309323482 13.5212923729393
347542.693131981 13.9017077252792
357320.647222047 14.2928258888819
367373.699560693 14.6949479824277
377709.589910827 15.1083835964331
388336.27579003 15.5334510316012
399261.938596989 15.9704775438795
410494.989910283 16.4197995964113
422044.077964396 16.8817631185759
433918.094307917 17.3567237723167
446126.180649069 17.8450472259628
458677.735893843 18.3471094357537
471582.423382129 18.8632969352851
484850.178327452 19.3940071330981
498491.215466006 19.9396486186402
512516.036920896 20.5006414768358
526935.440287643 21.0774176115057
541760.526947153 21.6704210778861
557002.710612593 22.2801084245037
572673.726116707 22.9069490446683
588785.638446366 23.5514255378547
605350.852031314 24.2140340812526
622382.120294223 24.8952848117689
639892.555469461 25.5957022187785
657895.638698086 26.3158255479234
676405.230406871 27.0562092162748
695435.580979334 27.8174232391734
715001.341726984 28.6000536690794
735117.576169259 29.4047030467704
755799.771630793 30.2319908652317
777063.851164993 31.0825540465997
798926.18581306 31.9570474325224
821403.607207919 32.8561442883167
844513.420532764 33.7805368213106
868273.417844168 34.7309367137667
892701.891770049 35.708075670802
917817.649593013 36.7127059837205
943640.027729919 37.7456011091968
970188.906618846 38.8075562647538
997484.726024861 39.8993890409944
1025548.50077644 41.0219400310577
1054401.83694461 42.1760734777845
1084066.94847728 43.3626779390914
1114566.6743016 44.582666972064
1145924.49590742 45.8369798362968
1178164.55542555 47.1265822170218
1211311.67421455 48.4524669685818
1245391.37197051 49.8156548788203
1280429.88637446 51.2171954549784
1316454.19329253 52.658167731701
1353492.02754445 54.1396811017781
1391571.90425639 55.6628761702555
1430723.14081447 57.228925632579
1470975.87943605 58.839035177442
1512361.11037589 60.4944444150355
1554910.69578536 62.1964278314144
1598657.39424283 63.9462957697133
1643634.88597423 65.7453954389693
1689877.79878317 67.595111951327
1737421.73471063 69.4968693884254
1786303.29744466 71.4521318977866
1836560.12050126 73.4624048200505
1888230.89619813 75.5292358479252
1941355.40544356 77.6542162177423
1995974.54836342 79.8389819345367
2052130.37578985 82.0852150315941
2109866.12163586 84.3946448654343
2169226.23618072 86.7690494472286
2230256.4202919 89.210256811676
2293003.66060982 91.7201464243928
2357516.26572243 94.3006506288973
2423843.90335763 96.9537561343051
2492037.63862202 99.681505544881
2562149.97331557 102.485998932623
2634234.88635222 105.369395454089
2708347.87531793 108.333915012717
2784545.99919772 111.381839967909
2862887.92230498 114.515516892199
2943433.95944659 117.737358377864
3026246.12235884 121.049844894354
3111388.16744978 124.455526697991
3198925.64488466 127.957025795386
3288925.94905258 131.557037962103
3381458.37045283 135.258334818113
3476594.14904105 139.063765961642
3574406.52907635 142.976261163054
3674970.81551142 146.998832620457
3778364.43196924 151.13457727877
3884666.98035084 155.386679214034
3993960.30212021 159.758412084808
4106328.54131334 164.253141652534
4221858.20932004 168.874328372802
4340638.25148833 173.625530059533
4462760.1156028 178.510404624112
4588317.82228943 183.532712891577
4717408.03740133 188.696321496053
4850130.14644105 194.005205857642
4986586.33107658 199.463453243063
5126881.64781024 205.075265912409
5271124.10886078 210.844964354431
5419424.76532117 216.776990612847
5571897.79265584 222.875911706234
5728660.57860353 229.146423144141
5889833.81355307 235.593352542123
6055541.58346201 242.22166333848
6225911.46538926 249.036458615571
6401074.6257158 256.042985028632
6581165.92112845 263.246636845138
6766324.00244499 270.6529600978
6956691.42136033 278.267656854413
7152414.74019584 286.096589607833
7353644.64473648 294.145785789459
7560536.06024264 302.421442409706
7773248.2707257 310.929930829028
7991945.04157965 319.677801663186
8216794.74566254 328.671789826501
8447970.49292555 337.918819717022
8685650.26368883 347.426010547553
8930017.04566709 357.200681826684
9181258.9748504 367.250358994016
9439569.48034852 377.582779213941
9705147.43331038 388.205897332415
9978197.30003336 399.127892001334
10258929.2993803 410.35717197521
10547559.5646251 421.902382585003
10844310.3098521 433.772412394086
11149410.0010371 445.976400041485
11463093.531941 458.523741277639
11785602.4049527 471.424096198108
12117184.9170202 484.687396680807
12458096.3508119 498.323854032477
12808599.1712571 512.343966850284
13168963.2276151 526.758529104602
13539465.9612303 541.57863844921
13920392.619132 556.815704765279
14312036.4736436 572.481458945745
14714699.0481708 588.587961926833
15128690.3493418 605.147613973671
15554329.1056788 622.17316422715
15991943.0129846 639.677720519385
16441868.9866334 657.674759465337
16904453.4209583 676.178136838331
17380052.4559379 695.202098237516
17869032.2513858 714.761290055433
18371769.2688538 734.870770754154
18888650.5614665 755.54602245866
19420074.0719104 776.802962876415
19966448.9388069 798.657957552275
20528195.8117045 821.127832468181
21105747.1749337 844.22988699735
21699547.6805731 867.981907222925
22310054.4907833 892.402179631332
22937737.6297722 917.50950519089
23583080.3456633 943.323213826533
24246579.482544 969.86317930176
24928745.8629818 997.149834519272
25630104.6813029 1025.20418725211
26351195.9079344 1054.04783631738
27092574.7051238 1083.70298820495
27854811.8543531 1114.19247417412
28638494.1957794 1145.53976783118
29444225.0800384 1177.76900320154
30272624.8327584 1210.90499331034
31124331.2321449 1244.97324928579
32000000 1280
};
\addplot [thick, steelblue31119180]
table {%
256 136.7278
512 127.2228
1024 129.2816
2048 148.2799
4096 146.4164
8192 150.9608
16384 152.881
32768 158.2081
65536 166.8456
131072 178.2599
262144 197.2738
524288 242.1888
1048576 239.5699
2097152 240.7576
4194304 239.0411
8388608 373.4915
16777216 705.9068
33554432 1430.342
};
\addlegendentry{\ptpart{}}
\addplot [thick, darkorange25512714]
table {%
256 4.594167
512 5.2814
1024 5.177833
2048 6.0549
4096 6.41308
8192 7.013193
16384 9.58728
32768 10.83776
65536 11.99247
131072 16.98291
262144 22.65143
524288 32.53746
1048576 54.67121
2097152 100.4991
4194304 190.8079
8388608 362.8952
16777216 701.0865
33554432 1384.874
};
\addlegendentry{\ptsingle{}}
\addplot [thick, darkolivegreen9912157]
table {%
256 132.8915
512 131.7979
1024 131.8337
2048 148.2148
4096 143.3956
8192 143.6767
16384 145.7476
32768 150.4719
65536 164.8515
131072 187.7152
262144 233.1864
524288 293.4696
1048576 289.0326
2097152 286.3335
4194304 287.4021
8388608 368.4751
16777216 708.1531
33554432 1515.922
};
\addlegendentry{\ptmany{}}
\addplot [thick, orchid227119194]
table {%
256 109.7324
512 108.8578
1024 110.4842
2048 109.7876
4096 119.4592
8192 123.8724
16384 123.5268
32768 125.7761
65536 130.6202
131072 157.6323
262144 188.9064
524288 195.6056
1048576 263.2719
2097152 326.6534
4194304 433.1751
8388608 611.9278
16777216 961.062
33554432 1785.071
};
\addlegendentry{\RMAmany{}}
\addplot [thick, crimson2143940]
table {%
256 40.47261
512 40.46953
1024 41.87881
2048 41.97347
4096 50.26061
8192 52.79659
16384 54.61669
32768 57.39695
65536 63.10083
131072 74.02655
262144 110.4319
524288 74.07639
1048576 72.80072
2097152 96.38475
4194304 180.361
8388608 350.8391
16777216 692.2133
33554432 1512.704
};
\addlegendentry{\RMAsingle{}}
\draw[->,draw=black,semithick] (axis cs:256,4.594167) -- (axis cs:256,136.7278);
\draw (axis cs:256,25.0629277368507) ++(2pt,-2pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{$\times 29.76$};
\end{axis}

\end{tikzpicture}


==> figures/results/TIME_congestion-32part-32thread-0sleep-32vci-0aggr.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkolivegreen9912157}{RGB}{99,121,57}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={msg size [\B]},
xmajorgrids,
xmin=142.024892424684, xmax=60481894.7252872,
xmode=log,
xtick style={color=black},
xtick={10,100,1000,10000,100000,1000000,10000000,100000000,1000000000},
xticklabels={
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{6}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{8}}\),
  \(\displaystyle {10^{9}}\)
},
y grid style={darkgray176},
ylabel={time [\mus]},
ymajorgrids,
ymin=1, ymax=2085.48471893518,
ymode=log,
ytick style={color=black},
ytick={0.1,1,10,100,1000,10000,100000},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{4}}\),
  \(\displaystyle {10^{5}}\)
}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.4]
(axis cs:256,19.3973519)
--(axis cs:256,19.0814081)
--(axis cs:512,19.0913307)
--(axis cs:1024,18.8778477)
--(axis cs:2048,19.1451831)
--(axis cs:4096,19.1696541)
--(axis cs:8192,19.2681772)
--(axis cs:16384,19.1166569)
--(axis cs:32768,19.3480861)
--(axis cs:65536,20.2128109)
--(axis cs:131072,21.8418928)
--(axis cs:262144,27.2803529)
--(axis cs:524288,43.8437857)
--(axis cs:1048576,67.7592254)
--(axis cs:2097152,113.9507988)
--(axis cs:4194304,199.8637451)
--(axis cs:8388608,368.77577)
--(axis cs:16777216,708.9312023)
--(axis cs:33554432,1387.7146629)
--(axis cs:33554432,1388.3693371)
--(axis cs:33554432,1388.3693371)
--(axis cs:16777216,709.4537977)
--(axis cs:8388608,369.30183)
--(axis cs:4194304,200.4322549)
--(axis cs:2097152,114.5188012)
--(axis cs:1048576,68.3665546)
--(axis cs:524288,44.3799143)
--(axis cs:262144,27.7667271)
--(axis cs:131072,22.2613672)
--(axis cs:65536,20.7152491)
--(axis cs:32768,19.7884339)
--(axis cs:16384,19.4613631)
--(axis cs:8192,19.8251228)
--(axis cs:4096,19.7134059)
--(axis cs:2048,19.6818169)
--(axis cs:1024,19.2212123)
--(axis cs:512,19.6978093)
--(axis cs:256,19.3973519)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.4]
(axis cs:256,4.84541017)
--(axis cs:256,4.68506983)
--(axis cs:512,4.78645754)
--(axis cs:1024,4.91708867)
--(axis cs:2048,5.33140089)
--(axis cs:4096,5.8525706)
--(axis cs:8192,6.32567172)
--(axis cs:16384,9.21353711)
--(axis cs:32768,10.114724)
--(axis cs:65536,11.5313105)
--(axis cs:131072,16.2172061)
--(axis cs:262144,22.1599914)
--(axis cs:524288,32.31473634)
--(axis cs:1048576,54.32738134)
--(axis cs:2097152,99.8830739)
--(axis cs:4194304,189.5970282)
--(axis cs:8388608,367.7304458)
--(axis cs:16777216,699.4333647)
--(axis cs:33554432,1389.1511847)
--(axis cs:33554432,1390.6028153)
--(axis cs:33554432,1390.6028153)
--(axis cs:16777216,700.2242353)
--(axis cs:8388608,368.4915542)
--(axis cs:4194304,189.8493718)
--(axis cs:2097152,100.2769261)
--(axis cs:1048576,54.51303866)
--(axis cs:524288,32.50938366)
--(axis cs:262144,22.3632686)
--(axis cs:131072,16.4593739)
--(axis cs:65536,11.7263695)
--(axis cs:32768,10.387696)
--(axis cs:16384,9.37250289)
--(axis cs:8192,6.51586228)
--(axis cs:4096,6.0796154)
--(axis cs:2048,5.51870511)
--(axis cs:1024,5.07969733)
--(axis cs:512,4.96468846)
--(axis cs:256,4.84541017)
--cycle;

\path [draw=darkolivegreen9912157, fill=darkolivegreen9912157, opacity=0.4]
(axis cs:256,4.17666412)
--(axis cs:256,3.99208188)
--(axis cs:512,3.9896582)
--(axis cs:1024,3.87758121)
--(axis cs:2048,4.5072536)
--(axis cs:4096,4.3816319)
--(axis cs:8192,5.3508946)
--(axis cs:16384,5.56033076)
--(axis cs:32768,6.5557417)
--(axis cs:65536,26.4412892)
--(axis cs:131072,26.600097)
--(axis cs:262144,27.1562826)
--(axis cs:524288,36.1099512)
--(axis cs:1048576,58.0903274)
--(axis cs:2097152,102.106028)
--(axis cs:4194304,187.6805986)
--(axis cs:8388608,357.8426947)
--(axis cs:16777216,697.3965246)
--(axis cs:33554432,1361.02886)
--(axis cs:33554432,1435.73914)
--(axis cs:33554432,1435.73914)
--(axis cs:16777216,697.8006754)
--(axis cs:8388608,358.3565053)
--(axis cs:4194304,188.1410014)
--(axis cs:2097152,102.634172)
--(axis cs:1048576,58.5584126)
--(axis cs:524288,36.7437288)
--(axis cs:262144,27.6331574)
--(axis cs:131072,27.140683)
--(axis cs:65536,27.0107708)
--(axis cs:32768,6.7887783)
--(axis cs:16384,5.74426924)
--(axis cs:8192,5.5317994)
--(axis cs:4096,4.5921541)
--(axis cs:2048,4.9116664)
--(axis cs:1024,4.03984479)
--(axis cs:512,4.2068358)
--(axis cs:256,4.17666412)
--cycle;

\path [draw=orchid227119194, fill=orchid227119194, opacity=0.4]
(axis cs:256,13.9145248)
--(axis cs:256,13.2891752)
--(axis cs:512,13.0823718)
--(axis cs:1024,13.0017866)
--(axis cs:2048,13.0840949)
--(axis cs:4096,12.655129)
--(axis cs:8192,12.8963598)
--(axis cs:16384,12.9203722)
--(axis cs:32768,13.1782008)
--(axis cs:65536,14.8523044)
--(axis cs:131072,19.4392191)
--(axis cs:262144,25.2790165)
--(axis cs:524288,35.5890604)
--(axis cs:1048576,55.8614961)
--(axis cs:2097152,99.5771347)
--(axis cs:4194304,183.8234886)
--(axis cs:8388608,354.2024036)
--(axis cs:16777216,694.8289378)
--(axis cs:33554432,1378.4022805)
--(axis cs:33554432,1378.7457195)
--(axis cs:33554432,1378.7457195)
--(axis cs:16777216,695.1430622)
--(axis cs:8388608,354.5589964)
--(axis cs:4194304,184.2423114)
--(axis cs:2097152,100.1319253)
--(axis cs:1048576,56.3219639)
--(axis cs:524288,36.1680396)
--(axis cs:262144,25.5937635)
--(axis cs:131072,19.8037209)
--(axis cs:65536,15.2309156)
--(axis cs:32768,13.5126992)
--(axis cs:16384,13.2313278)
--(axis cs:8192,13.5532602)
--(axis cs:4096,13.001571)
--(axis cs:2048,13.3939251)
--(axis cs:1024,13.2656734)
--(axis cs:512,13.4133682)
--(axis cs:256,13.9145248)
--cycle;

\path [draw=crimson2143940, fill=crimson2143940, opacity=0.4]
(axis cs:256,43.7187218)
--(axis cs:256,42.8951982)
--(axis cs:512,40.1004086)
--(axis cs:1024,43.2018209)
--(axis cs:2048,42.9269027)
--(axis cs:4096,49.2582616)
--(axis cs:8192,54.5698794)
--(axis cs:16384,55.997735)
--(axis cs:32768,57.5150052)
--(axis cs:65536,63.115533)
--(axis cs:131072,81.609841)
--(axis cs:262144,113.457108)
--(axis cs:524288,70.371513)
--(axis cs:1048576,63.7449038)
--(axis cs:2097152,96.0599344)
--(axis cs:4194304,189.6331305)
--(axis cs:8388608,371.9228085)
--(axis cs:16777216,733.0435287)
--(axis cs:33554432,1520.06834)
--(axis cs:33554432,1545.88166)
--(axis cs:33554432,1545.88166)
--(axis cs:16777216,733.2806713)
--(axis cs:8388608,372.6297915)
--(axis cs:4194304,189.9058695)
--(axis cs:2097152,96.3699856)
--(axis cs:1048576,65.6399962)
--(axis cs:524288,73.052247)
--(axis cs:262144,117.740892)
--(axis cs:131072,85.173279)
--(axis cs:65536,65.367307)
--(axis cs:32768,59.1471348)
--(axis cs:16384,58.196365)
--(axis cs:8192,56.2152606)
--(axis cs:4096,50.4556384)
--(axis cs:2048,43.6877173)
--(axis cs:1024,43.8876591)
--(axis cs:512,40.7265714)
--(axis cs:256,43.7187218)
--cycle;

\addplot [thick, black, dash pattern=on 12.8pt off 3.2pt on 2pt off 3.2pt, forget plot]
table {%
128000 5.12
131601.221226231 5.26404884904925
135303.76115809 5.4121504463236
139110.470350835 5.56441881403342
143024.279558792 5.72097118235169
147048.201991711 5.88192807966843
151185.335634614 6.04741342538458
155438.865632914 6.21755462531655
159812.066744621 6.39248266978485
164308.305861564 6.57233223446255
168931.044601523 6.75724178406091
173683.841973307 6.94735367893229
178570.357116805 7.1428142846722
183594.352120123 7.34377408480493
188759.694915992 7.55038779663968
194070.362259651 7.76281449038605
199530.442790525 7.98121771162101
205144.14018003 8.2057656072012
210915.776367946 8.43663105471784
216849.794889847 8.67399179559389
222950.764298138 8.91803057192552
229223.381679349 9.16893526717395
235672.476270381 9.42689905081525
242303.013176501 9.69212052706006
249120.097193932 9.96480388775727
256128.976739991 10.2451590695996
263335.047893811 10.5334019157524
270743.858550732 10.8297543420293
278361.11269358 11.1344445077432
286192.674784124 11.4477069913649
294244.574278065 11.7697829711226
302523.010267077 12.1009204106831
311034.35625143 12.4413742500572
319785.165046898 12.7914066018759
328782.173829717 13.1512869531887
338032.309323482 13.5212923729393
347542.693131981 13.9017077252792
357320.647222047 14.2928258888819
367373.699560693 14.6949479824277
377709.589910827 15.1083835964331
388336.27579003 15.5334510316012
399261.938596989 15.9704775438795
410494.989910283 16.4197995964113
422044.077964396 16.8817631185759
433918.094307917 17.3567237723167
446126.180649069 17.8450472259628
458677.735893843 18.3471094357537
471582.423382129 18.8632969352851
484850.178327452 19.3940071330981
498491.215466006 19.9396486186402
512516.036920896 20.5006414768358
526935.440287643 21.0774176115057
541760.526947153 21.6704210778861
557002.710612593 22.2801084245037
572673.726116707 22.9069490446683
588785.638446366 23.5514255378547
605350.852031314 24.2140340812526
622382.120294223 24.8952848117689
639892.555469461 25.5957022187785
657895.638698086 26.3158255479234
676405.230406871 27.0562092162748
695435.580979334 27.8174232391734
715001.341726984 28.6000536690794
735117.576169259 29.4047030467704
755799.771630793 30.2319908652317
777063.851164993 31.0825540465997
798926.18581306 31.9570474325224
821403.607207919 32.8561442883167
844513.420532764 33.7805368213106
868273.417844168 34.7309367137667
892701.891770049 35.708075670802
917817.649593013 36.7127059837205
943640.027729919 37.7456011091968
970188.906618846 38.8075562647538
997484.726024861 39.8993890409944
1025548.50077644 41.0219400310577
1054401.83694461 42.1760734777845
1084066.94847728 43.3626779390914
1114566.6743016 44.582666972064
1145924.49590742 45.8369798362968
1178164.55542555 47.1265822170218
1211311.67421455 48.4524669685818
1245391.37197051 49.8156548788203
1280429.88637446 51.2171954549784
1316454.19329253 52.658167731701
1353492.02754445 54.1396811017781
1391571.90425639 55.6628761702555
1430723.14081447 57.228925632579
1470975.87943605 58.839035177442
1512361.11037589 60.4944444150355
1554910.69578536 62.1964278314144
1598657.39424283 63.9462957697133
1643634.88597423 65.7453954389693
1689877.79878317 67.595111951327
1737421.73471063 69.4968693884254
1786303.29744466 71.4521318977866
1836560.12050126 73.4624048200505
1888230.89619813 75.5292358479252
1941355.40544356 77.6542162177423
1995974.54836342 79.8389819345367
2052130.37578985 82.0852150315941
2109866.12163586 84.3946448654343
2169226.23618072 86.7690494472286
2230256.4202919 89.210256811676
2293003.66060982 91.7201464243928
2357516.26572243 94.3006506288973
2423843.90335763 96.9537561343051
2492037.63862202 99.681505544881
2562149.97331557 102.485998932623
2634234.88635222 105.369395454089
2708347.87531793 108.333915012717
2784545.99919772 111.381839967909
2862887.92230498 114.515516892199
2943433.95944659 117.737358377864
3026246.12235884 121.049844894354
3111388.16744978 124.455526697991
3198925.64488466 127.957025795386
3288925.94905258 131.557037962103
3381458.37045283 135.258334818113
3476594.14904105 139.063765961642
3574406.52907635 142.976261163054
3674970.81551142 146.998832620457
3778364.43196924 151.13457727877
3884666.98035084 155.386679214034
3993960.30212021 159.758412084808
4106328.54131334 164.253141652534
4221858.20932004 168.874328372802
4340638.25148833 173.625530059533
4462760.1156028 178.510404624112
4588317.82228943 183.532712891577
4717408.03740133 188.696321496053
4850130.14644105 194.005205857642
4986586.33107658 199.463453243063
5126881.64781024 205.075265912409
5271124.10886078 210.844964354431
5419424.76532117 216.776990612847
5571897.79265584 222.875911706234
5728660.57860353 229.146423144141
5889833.81355307 235.593352542123
6055541.58346201 242.22166333848
6225911.46538926 249.036458615571
6401074.6257158 256.042985028632
6581165.92112845 263.246636845138
6766324.00244499 270.6529600978
6956691.42136033 278.267656854413
7152414.74019584 286.096589607833
7353644.64473648 294.145785789459
7560536.06024264 302.421442409706
7773248.2707257 310.929930829028
7991945.04157965 319.677801663186
8216794.74566254 328.671789826501
8447970.49292555 337.918819717022
8685650.26368883 347.426010547553
8930017.04566709 357.200681826684
9181258.9748504 367.250358994016
9439569.48034852 377.582779213941
9705147.43331038 388.205897332415
9978197.30003336 399.127892001334
10258929.2993803 410.35717197521
10547559.5646251 421.902382585003
10844310.3098521 433.772412394086
11149410.0010371 445.976400041485
11463093.531941 458.523741277639
11785602.4049527 471.424096198108
12117184.9170202 484.687396680807
12458096.3508119 498.323854032477
12808599.1712571 512.343966850284
13168963.2276151 526.758529104602
13539465.9612303 541.57863844921
13920392.619132 556.815704765279
14312036.4736436 572.481458945745
14714699.0481708 588.587961926833
15128690.3493418 605.147613973671
15554329.1056788 622.17316422715
15991943.0129846 639.677720519385
16441868.9866334 657.674759465337
16904453.4209583 676.178136838331
17380052.4559379 695.202098237516
17869032.2513858 714.761290055433
18371769.2688538 734.870770754154
18888650.5614665 755.54602245866
19420074.0719104 776.802962876415
19966448.9388069 798.657957552275
20528195.8117045 821.127832468181
21105747.1749337 844.22988699735
21699547.6805731 867.981907222925
22310054.4907833 892.402179631332
22937737.6297722 917.50950519089
23583080.3456633 943.323213826533
24246579.482544 969.86317930176
24928745.8629818 997.149834519272
25630104.6813029 1025.20418725211
26351195.9079344 1054.04783631738
27092574.7051238 1083.70298820495
27854811.8543531 1114.19247417412
28638494.1957794 1145.53976783118
29444225.0800384 1177.76900320154
30272624.8327584 1210.90499331034
31124331.2321449 1244.97324928579
32000000 1280
};
\addplot [thick, steelblue31119180]
table {%
256 19.23938
512 19.39457
1024 19.04953
2048 19.4135
4096 19.44153
8192 19.54665
16384 19.28901
32768 19.56826
65536 20.46403
131072 22.05163
262144 27.52354
524288 44.11185
1048576 68.06289
2097152 114.2348
4194304 200.148
8388608 369.0388
16777216 709.1925
33554432 1388.042
};
\addlegendentry{\ptpart{}}
\addplot [thick, darkorange25512714]
table {%
256 4.76524
512 4.875573
1024 4.998393
2048 5.425053
4096 5.966093
8192 6.420767
16384 9.29302
32768 10.25121
65536 11.62884
131072 16.33829
262144 22.26163
524288 32.41206
1048576 54.42021
2097152 100.08
4194304 189.7232
8388608 368.111
16777216 699.8288
33554432 1389.877
};
\addlegendentry{\ptsingle{}}
\addplot [thick, darkolivegreen9912157]
table {%
256 4.084373
512 4.098247
1024 3.958713
2048 4.70946
4096 4.486893
8192 5.441347
16384 5.6523
32768 6.67226
65536 26.72603
131072 26.87039
262144 27.39472
524288 36.42684
1048576 58.32437
2097152 102.3701
4194304 187.9108
8388608 358.0996
16777216 697.5986
33554432 1398.384
};
\addlegendentry{\ptmany{}}
\addplot [thick, orchid227119194]
table {%
256 13.60185
512 13.24787
1024 13.13373
2048 13.23901
4096 12.82835
8192 13.22481
16384 13.07585
32768 13.34545
65536 15.04161
131072 19.62147
262144 25.43639
524288 35.87855
1048576 56.09173
2097152 99.85453
4194304 184.0329
8388608 354.3807
16777216 694.986
33554432 1378.574
};
\addlegendentry{\RMAmany{}}
\addplot [thick, crimson2143940]
table {%
256 43.30696
512 40.41349
1024 43.54474
2048 43.30731
4096 49.85695
8192 55.39257
16384 57.09705
32768 58.33107
65536 64.24142
131072 83.39156
262144 115.599
524288 71.71188
1048576 64.69245
2097152 96.21496
4194304 189.7695
8388608 372.2763
16777216 733.1621
33554432 1532.975
};
\addlegendentry{\RMAsingle{}}
\draw[->,draw=black,semithick] (axis cs:256,4.76524) -- (axis cs:256,19.23938);
\draw (axis cs:256,9.57498110448266) ++(2pt,-2pt) node[
  scale=0.833333333333333,
  fill=white,
  draw=white,
  line width=0.4pt,
  inner sep=2.4pt,
  anchor=base west,
  text=black,
  rotate=0.0
]{$\times 4.04$};
\end{axis}

\end{tikzpicture}

